Active Learning of Abstract Plan Feasibility

Long horizon sequential manipulation tasks are effectively addressed hierarchically: at a high level of abstraction the planner searches over abstract action sequences, and when a plan is found, lower level motion plans are generated. Such a strategy hinges on the ability to reliably predict that a feasible low level plan will be found which satisfies the abstract plan. However, computing Abstract Plan Feasibility (APF) is difficult because the outcome of a plan depends on real-world phenomena that are difficult to model, such as noise in estimation and execution. In this work, we present an active learning approach to efficiently acquire an APF predictor through task-independent, curious exploration on a robot. The robot identifies plans whose outcomes would be informative about APF, executes those plans, and learns from their successes or failures. Critically, we leverage an infeasible subsequence property to prune candidate plans in the active learning strategy, allowing our system to learn from less data. We evaluate our strategy in simulation and on a real Franka Emika Panda robot with integrated perception, experimentation, planning, and execution. In a stacking domain where objects have non-uniform mass distributions, we show that our system permits real robot learning of an APF model in four hundred self-supervised interactions, and that our learned model can be used effectively in multiple downstream tasks.

==> sections/backup/method_backup.tex <==
Collecting data on real robot platforms is both time and cost-intensive.
In addition, when considering the space of sequential actions with multiple object interactions, the search space is prohibitively large.
In order to minimize the amount of data needed to learn the \apf{} model, we take an information theoretic approach to active learning \cite{houlsby_bayesian_2011}.
Concretely, we maintain a distribution over model parameters that are consistent with the data we have observed so far.
Our objective is to select new data that minimize the entropy over this distribution as fast as possible.
Efficient active learning requires: (1) a model class that captures uncertainty over model parameters, (2) a way to calculate expected information gain between unlabeled plans and model parameters, and (3) a method of generating potentially informative plans.
We discuss each of these in turn.

\subsection{Abstract plan feasibility model}
\label{sec:method-apf-model}

Our \apf{} model, $\Pr(\feas \mid \ba; \Theta)$, aims to capture the uncertainty in the underlying stochastic process of predicting the feasibility of abstract action sequences.
This uncertainty can be attributed to phenomena such as the robot's motor capabilities, errors in perception, or unmodeled behaviors of the planning process, and is referred to as {\em aleatoric uncertainty}. 
Our goal is to learn parameters $\Theta$ such that this uncertainty is adequately captured and our model can be leveraged, along with a low level planner, to achieve a goal.

We take a Bayesian approach to learning the model parameters, and maintain a distribution over the parameter space, $\Pr(\Theta)$.
This distribution aims to capture the uncertainty we have regarding the accuracy of our predictions, and is referred to as {\em epistemic uncertainty}. 
In general, for complex model classes such as our proposed neural network classifier, an explicit representation of $\Pr(\Theta \mid \Data)$ for training data $\Data$ is difficult to construct or update with new data.
We therefore follow the strategy of \cite{beluch_power_2018} and represent this uncertainty with an ensemble of $N$ models, $\bm{\theta}=(\theta_1, \ldots, \theta_N)$, where ${\theta_i} \in \mathbb{R}^{d}$ and ${\bm\theta} \in \mathbb{R}^{Nd}$. 
Initial parameters are drawn independently at random and are updated to incorporate new data via gradient descent.

%Because our objective is to learn the \apf{} model from as few data samples as possible, it is critical that we make our {\em epistemic uncertainty} about the model explicit.  We represent our particular model using a parameter vector $\theta$ in the space of possible \apf{} models $\Theta$, and the prediction of a particular model is $\Pr(\feas \mid \ba; \theta)$. If we were to maintain a distribution on the model parameter space, $\Pr(\Theta)$, the entropy of that distribution would be the {\em epistemic uncertainty} of our model.

%%At the same time, we desire a model class that is flexible enough to learn about plan feasibility in the real world. 
%However, in general, for complex model classes such as our proposed neural network classifier, an explicit representation of $\Pr(\Theta \mid \Data)$ for training data $\Data$ is too difficult to construct or update with new data.  We therefore follow the strategy of \cite{beluch_power_2018} and represent this uncertainty using an ensemble of $N$ models, parameterized by $(\theta_1, \ldots, \theta_N)$. Initial parameters are drawn independently at random and are updated to incorporate new data via gradient descent.

%% Although domain-specific models could be applied, in this work we consider neural networks architectures to maintain generality. This decision highlights the data-efficiency of the \bald{} acquisition strategy; our model achieves acceptable performance on downstream tasks after collecting only 400 towers in the experimentation phase.

The design of the models in the ensemble is selected to match the underlying structure of the prediction problem.  Importantly, the length of plans for which we require predictions varies during both the experimentation and execution phases.  For this reason, we use {\em graph neural networks} ({\sc gnn}s), which make predictions based on aggregations of local properties and relations among the input entities, and exploit parameter tying to model global properties of collections of objects of arbitrary size using a fixed-dimensional parameterization $\Theta$.  For a detailed description of {\sc gnn}s, see the overview by \cite{zhou2018graph}.
More details about the specific architecture we use can be found in Section \ref{sec:imp-learning}.

%%We take advantage of the {\em infeasible sub-sequence} property of the \apf{} problem to design a special connectivity structure for our {\sc gnn} models.  As shown in figure~\ref{fig:graph_network}, the node corresponding to action $a_i$ is connected to each node representing $a_j$ for $1 \leq j < i$.  This encodes the structural property that the feasibility of step $i$ in the plan depends on all previous actions.  To make a prediction, an encoding of $\ba$ is fed into the network, some number of rounds of message passing is performed on the graph using the local neural network models $\theta$, and the average activation level of each node is computed and passed through a sigmoidal transformation to obtain a prediction $\Pr(\feas \mid \ba)$.
%\lpknote{We might want to put more details in here?}

\subsection{Entropy reduction}

Following \cite{mackay1992objective, cohn1996active}, we guide our active learning by picking a sequence of data $\Data$ that maximally reduces the entropy of $\Pr(\Theta \mid \Data)$. The general problem of designing a sequence of experiments to minimize entropy --- or equivalently, maximize information gain --- is a difficult sequential decision-making problem.  Fortunately, due to sub-modularity of the objective, a \emph{myopic} approach that considers only the next experiment to conduct can be shown to be a good approximation to the optimal experimentation strategy \cite{Nemhauser1978submodular}. 

Given a model distribution $\Pr(\Theta \mid \Data)$ that depends on the data we have seen so far, $\Data$, we choose the action sequence $\ba \in \A$ that reduces the entropy of the posterior distribution as much as possible: 
% \inote{this seems to imply that we've already marginalized out $\phi$? We may need to have $\ent(\Theta \mid \Data, \ba, \phi)$. I just went back to looked at the original paper, and they just drop the form with the expectation over $\phi$ with no explanation...}
\begin{equation}\label{eq:theta_entropy_objective2}
\ba^* = \argmax{\ba\in\A} \ent(\Theta \mid \Data) - \ent(\Theta \mid \Data, \ba). 
\end{equation}
While the agent can select the plan, $\ba$, to experiment with, it cannot select the outcome $\feas$, so to compute this quantity, we have to take an expectation over the outcome, using our current model distribution:
\[\ent(\Theta \mid \Data, \ba) = \expect{\feas \sim \Pr(\cdot \mid \Data, \ba)} \left[ \ent(\Theta \mid \Data, \ba, \feas) \right].\]
% where 
% \[\Pr(\feas \mid \Data, \ba) = \int_\theta \Pr(\feas \mid \ba; \theta) \Pr(\theta \mid \Data).\]

Estimating the entropy over a high-dimensional parameter space is expensive, so we follow the approach of~\citet{houlsby_bayesian_2011} to reformulate the objective in (\ref{eq:theta_entropy_objective2}) as 
\begin{align}\label{eq:y_entropy_objective2}
\ba^* &= \argmax{\ba\in\A} \info(\Feas : \Theta \mid \Data, \ba) \\
&= \argmax{\ba\in\A} \ent(\Feas \mid \Data, \ba) - 
                          \expect{\Theta \sim \Pr(\cdot \mid \Data)} \left[ \ent(\Feas \mid \ba; \Theta) \right],
\end{align}
allowing the computation of entropies to take place in the typically lower-dimensional label space, $\Feas$. This is known as the {\em Bayesian Active Learning by Disagreement}, or \bald{}, objective.

In addition to improved efficiency, the \bald{} objective invites an appealing interpretation: maximizing the first term encourages selecting an $\ba$ that our model is overall uncertain about, and minimizing the second term encourages selecting an $\ba$ for which the individual models in $\bm\theta$ can make confident predictions about the outcome $\feas$.  If we think of the overall uncertainty as a combination of \emph{epistemic} and \emph{aleatoric uncertainty}, then this objective seeks an example with high overall uncertainty and low \emph{aleatoric uncertainty}, which therefore has high \emph{epistemic uncertainty}.  In other words, if the various possible models in $\Pr(\Theta \mid \Data)$ are individually confident but about differing outcomes, then observing the $\feas$ value corresponding to $\ba$ is likely to prove some of those outcomes incorrect.

Using an ensemble of equally weighted parameter vectors $\theta_1, \ldots, \theta_N$ to represent $\Pr(\Theta \mid \Data)$ allows us to compute a global feasibility prediction
\[
\widehat{\Pr}(\Feas = \feas \mid \ba; \Theta) = \frac{1}{N} \sum_{i=1}^N \Pr(\Feas = \feas \mid \ba; \theta_i)
\]
as well as find the experiment that optimizes the estimated \bald{} objective in the form \begin{equation}\label{eq:final-criterion}
\ba^* = \argmax{\ba\in\A} \ent(\widehat{\Pr}(\Feas \mid \ba; \Theta)) - 
                          \frac{1}{N}\sum_{i=1}^N \ent(\Pr(\Feas \mid \ba; \theta_i)).
                          \end{equation}
                          
\subsection{Sampling Strategies}
\label{sec:exp-design}

Now that we have established an informational score for experiments, we consider several sampling strategies for optimizing over $\A$, the set of plans up to a fixed length $L$.

Maximizing the \bald{} objective over the entire set $\A$ is difficult because we need to consider all discrete plans up to length $L$, as well as all possible assignments to each continuous abstract action parameter. Additionally, information gain is in general non-convex. One strategy we consider is uniformly sampling complete plans from $\A$ and scoring the samples. We call this the \complete{} strategy. 
\begin{equation}
\argmax{\ba \in \A}  \text{\bald{}}(\ba)
\end{equation}

Unfortunately, to achieve a consistent sampling density, the number of required samples scales exponentially with the length of the plan. Additionally, this strategy might generate most of its samples in the infeasible part of the space.

%We observe that the \emph{infeasible sub-sequence property} provides a strong constraint on the set of feasible plans: sequence $\as$ is only feasible if all of its prefixes are also feasible. As such, when calculating the feasibility of a plan, we use our model recursively, to determine the likelihood of success given each subsequence is successful.
%The probability that the plan is feasible is:
% \begin{equation}
%     \Pr(\Phi=\bm1|a_{1:L}, \Theta) = \prod\limits_{l=1}^L \Pr(\Phi=\bm1|a_{1:l}; \Theta),
% \end{equation}

We observe that the \emph{infeasible sub-sequence property} provides a strong constraint on the set of feasible plans: sequence $\as$ is only feasible if all of its prefixes are also feasible. As such, the model can learn the probability a specific action is feasible instead of the entire plan. If we denote the feasibility of each individual action as $\Phi_l$, then the probability that the plan is feasible is:
\begin{equation}
    \Pr(\Phi_{1:L}|\ba, \Theta) = \prod\limits_{l=1}^L \Pr(\Phi_l|a_{1:l}, \Phi_{1:l-1} = \bm1; \Theta),
\end{equation}
where $\Phi_l$ represents whether action $a_l$ is feasible and we use the subscript $1:L$ to refer to a sequence of variables.

Now each plan will return multiple feasibility labels and we can select plans where multiple of these labels will be informative.
Importantly, we need to take into account the probability a specific action will be attempted (i.e., that the plan was successful up until that action).
%Fortunately as our learned \apf{} model improves, we can leverage its predictions to evaluate the likelihood of successfully collecting an observation in new experiments. 
We call this the \sequential{} strategy.

\begin{equation}
\argmax{\as \in \A} \sum_{i=2}^n \widehat{\Pr}(\Feas_{1:i-1} = \bm1 \mid a_{1:i-1}; \Theta) \text{\bald{}}(a_i)
\end{equation}

We implement the \sequential{} approach naively by sampling and scoring entire plans. Like  \complete{}, this method requires exponentially more samples for longer plans, however, in the domain we considered, a sampling approach was acceptable as we had a relatively short plan horizon. In future work we hope to extend this strategy to a search-based method which prunes candidate plans by their feasibility.

We also consider a third strategy which uses the \emph{infeasible sub-sequence property} to bias our sampling towards plans that are much more likely to be feasible, and therefore informative. We only consider sequences $\as$ for which the prefix $(a_1, \ldots, a_{n-1})$ together with result $\feas = 1$ are in the current data set $\Data$.  We call this the \incremental{} strategy.

\begin{equation}
\argmax{a_n \in \A} \mathbbm{1}_{(a_{1:n-1}, \feas=1) \in \Data} \text{\bald{}}(a_n)
\end{equation}

Although this strategy finds more feasible plans than \complete{}, it also requires that the robot re-use plan prefixes, so we do not gather novel observations when repeating a plan prefix. Constraining our experiments to build on previously feasible plans may be overly restrictive. 
One might also consider a \greedy{} approach, in which we select the action $a_n$ which maximizes the \bald{} objective, given that we have already constructed $a_{1:n-1}$.

==> sections/ideas.tex <==
\begin{enumerate}
    \item How to learn models on a robot (what's presented above)
    \item How to do active learning on graph NNs. Right now the only thing that's different from the original BALD paper is that we're using an ensemble instead of mc-dropout. If we could come up with a way to exploit the graph structure in optimizing the bald score we could make that a focus of our paper.
    \item Active learning of unknown unknowns. This isn't great because it's a bit out of left field, and the active learning and the joint learning of latents and dynamics don't presently overlap all that much.
\end{enumerate}

==> sections/old_sections/active.tex <==
% general intro about active learning with ensembles
Collecting data on real robot platforms is both time and cost-intensive.
In addition, when considering the space of sequential actions with multiple object interactions, the search space is prohibitively large.
Thus, we take an active learning approach in the hopes of being substantially more data efficient than a naive strategy.
Our acquisition strategy consists of searching the input space to find where our model is most uncertain.
Our strategy also limits the search space of possible inputs by only considering feasible actions.
The acquisition strategy we use depends on a posterior distribution over model parameters given the data seen so far, $p(\bm{\theta}|D)$.
We model this distribution my maintaining an ensemble of models, and using the outputs of these models as a distribution over the true model parameters.
In this section we will describe in detail how this ensemble of models is used to guide data collection, and how we specify feasibility in the action space.

\subsection{BALD Acquisition with an Ensemble of Models}
\label{sec:bald}

Our objective is to learn the global dynamics $p(\bm{y} | \bm{x} ; \bm{\theta})$  with parameters $\bm{\theta}$ in as few interactions as possible.
Denoting the posterior distribution over our parameters given our observations by $p(\bm{\theta} |D)$, we formalize our ``few interactions'' objective as selecting observations which maximally reduce the uncertainty over $p(\bm{\theta} |D)$, quantified by Shannon entropy $H(\bm{\theta} | D)$. This can also be seen as selecting interactions which reduce the the size of the hypothesis space as quickly as possible.

\begin{equation}
    \underset{D}{\text{argmin}} \  H(\bm{\theta} | D)
\end{equation}

While finding the set of interactions that jointly minimize the entropy of the parameters is difficult, entropy is submodular and monotone, which means that a greedy sequential selection will be within $(1 - \frac{1}{e})$ of optimal \cite{Nemhauser1978submodular}. 

\begin{equation}
    \underset{\bm{x}, \bm{y}}{\text{argmax}} \  H(\bm{\theta} | D) - H(\bm{\theta} | \bm{x}, \bm{y}, D)
\end{equation}

While the agent can put the world in an initial state $\bm{x}$, it cannot select the outcome $\bm{y}$. Fortunately, we have a prediction of $\bm{y}$ using our learned dynamics dynamics:

\begin{equation}
    \underset{\bm{x}}{\text{argmax}} \  H(\bm{\theta} | D) - \mathbb{E}_{\bm{y} \sim p(\cdot | \bm{x}, D)}  \left [ H(\bm{\theta} | \bm{x}, \bm{y}, D) \right ]
    \label{eq:theta_entropy_objective}
\end{equation}

Computing entropy is subject to the curse of dimensionality, and the parameter space is often high-dimensional. To address this, Houlsby et. al. \cite{houlsby_bayesian_2011} show that Equation \ref{eq:theta_entropy_objective} is equivalent to 

\begin{equation}
    \underset{\bm{x}}{\text{argmax}} \  H(\bm{y} | \bm{x}, D) - \mathbb{E}_{\bm{\theta} \sim p(\cdot |D)}  \left [ H(\bm{y} | \bm{x}, \bm{\theta}) \right ]
    \label{eq:y_entropy_objective}
\end{equation}

 allowing the computation of entropies to take place in the typically lower-dimensional label-space. In addition to saving compute, Equation \ref{eq:y_entropy_objective} invites an appealing interpretation: the left term encourages selecting an $\bm{x}$ that our model is overall uncertain about, $\bm{y}$, and the right term encourages selecting an $\bm{x}$ where parameters sampled from the posterior are confident about different outcomes. In other words, if the various possible models in the posterior distribution over $\bm{\theta}$ are individually confident but about differing outcomes, then observing $\bm{y}$ is likely to prove some of those outcomes incorrect.

In our work, our global dynamics model is represented by an ensemble of $N$ models, each with their own parameters, $\bm{\theta_i}$. 
At inference time, we make predictions by averaging over these models

\begin{equation}
    \hat{\bm{y}} = p(\bm{y} | \bm{x}, \bm{\theta}) = \frac{1}{N} \sum_{i=1}^{i=N} \hat{\bm{y}}_i
\end{equation}
\begin{equation}
    \hat{\bm{y}}_i = p(\bm{y}|\bm{x}, \bm{\theta_i})
\end{equation}

When evaluating the BALD objective in Equation \ref{eq:y_entropy_objective} with an ensemble of models, the first term represents the entropy over our ensemble's prediction. 

\begin{equation}
    H(\bm{y} | \bm{x}, D) = H(\hat{\bm{y}}|\bm{x}, D, \bm{\theta})
\end{equation}


The second term represents the average entropy of our individual model predictions.

\begin{equation}
    \mathbb{E}_{\bm{\theta} \sim p(\cdot |D)}  \left [ H(\bm{y} | \bm{x}, \bm{\theta}) \right ] = \frac{1}{N} \sum_{i=1}^{i=N} H(\hat{\bm{y}}_i|\bm{x}, \bm{\theta_i})
\end{equation}

\subsection{Feasible Action Acquisition}
\label{sec:acquisition}

Active learning is a viable approach to limiting the amount of labeled data needed to learn a global dynamics model. 
Typically active learning involves selecting useful data from a given pool of unlabeled inputs.
In long-horizon manipulation problems, randomly generating a pool of unlabeled data is unlikely to produce useful inputs.
Given the large search space, more work is needed to ensure that the active learner is able to generate a pool of unlabeled data that is useful.
As mentioned, the input to our model is a set of desired object states.
In our work, we leverage the fact that much of this input space is actually inaccessible to the robot. 
If we naively performed a random search for sequences of actions, or object placements, we would end up considering sequences in which the robot fails to achieve the desired world state early on in the sequence.
Thus, we limit our search to sequences which differ from successful sequences in the existing labeled dataset by just one action.
Therefore the robot is not considering long sequences which it most likely cannot attempt, but rather just incrementally trying to add a single action to sequences that are feasible.
We also assume that all sequences consisting of just one action will be successful.
The details of our active learning method are given in Algorithm \ref{alg:active}.

\begin{algorithm}
\caption{Active Learning Algorithm}
\begin{algorithmic}[1]
    \Procedure{ActiveLearning}{$model, actions$}
    \State $D_{train} = \{\}$
    \Repeat
        \State $D_{pool} =  \textproc{GeneratePool}(D_{train}, actions)$
        \State $D_{BALD} = \textproc{BALD}(model, D_{pool})$
        \Comment{Eq. \ref{eq:y_entropy_objective}}
        \ForAll{$\bm{x} \in D_{BALD}$}
            \State $\bm{y} = \textproc{PlanAndExecute}(\bm{x})$
            \State $ D_{train} = D_{train} \cup {(\bm{x}, \bm{y})}$
        \EndFor
        \State $model.\textproc{Train}(D_{train})$
    \Until{}
\end{algorithmic}
\begin{algorithmic}[1]
    \Procedure{GeneratePool}{$D_{train}, actions$}
    \State $D_{pool} = \{\}$
    \ForAll{$action \in actions$}
        \State $D_{pool} = D_{pool} \cup \{action\}$
    \EndFor
    \ForAll{$(\bm{x},\bm{y}) \in D_{train}$}
        \ForAll{$action \in actions$}
            \If{$\textproc{Success}(\bm{y})$}
                \State $D_{pool} = D_{pool} \cup \{\bm{x} \cup action\}$
            \EndIf
        \EndFor
    \EndFor
\end{algorithmic}
\label{alg:active}
\end{algorithm}

==> sections/old_sections/domain.tex <==
The domain used in this work is one in which a robot interacts with a set of known cuboid objects with non-uniform centers of mass.
Each object has state $\bm{o} = (m, \bm{d}, \bm{c}, \bm{p})$, where $m \in \mathbb{R}$ is the mass of the object, $\bm{d} \in \mathbb{R}^3$ are the dimensions of the object, $\bm{c} \in \mathbb{R}^3$ is the center of mass relative to the geometric center of the object, and $\bm{p} \in SE(3)$ is the position of the object in the world frame.
A state, $\bm{x}$, is defined by a set of object states.

\subsection{Local Interactions}

We leverage a TAMP planner, PDDLStream \cite{garrett2020pddlstream}, to allow the robot to plan for interactions with individual objects.
We specify a planning model that reasons about picking and placing individual objects.
Given a state, $\bm{x}$, the planner returns a sequence of pick, place, and move actions that attempt to achieve it.
% Not sure how much detail we need to go into here...
\textcolor{red}{We are planning on giving brief PDDL descriptions of the actions (pick, place, move, move-free) we use, but are open to suggestions on if that is necessary.}

\subsection{Global Dynamics}

We consider the \emph{constructability} of towers in this work, as show in Figure \ref{fig:constructability}.
This is different from stability in that towers can be stable, but impossible for a single-armed manipulator to construct.


\begin{figure}
    \centering
    \includegraphics[clip, trim={0 0cm 0 0cm}, width=0.8\columnwidth]{figures/constructability.png}
    \caption{The size and placement of the black dot on each block corresponds to the mass and center of mass, respectively. The tower shown on the left is stable but not constructable. After placing the yellow block, it would fall off of the red block preventing the robot from building any further. However, if one were to hold the yellow block in place while placing the blue block, the weight of the blue block would hold the tower stably in place. The tower on the right is both constructable and stable.}
    \label{fig:constructability}
\end{figure}

\subsection{Graph Network Connectivity}
\label{sec:gn-con}

The base model used in our ensemble of models is a Graph Neural Network. 
A single graph structure is used to represent a tower, where each node corresponds to a block, and each edge corresponds to a connection between blocks.
We refer to \cite{zhou2018graph} for more details on graph networks.
In our work, the connectivity of the graph corresponds to the true underlying stability model.
When analytically determining the stability of a tower, one iteratively consider each subtower starting with the top block.
If the combined center of mass of a subtower lies within the contact patch of the surface below it, then it is stable.
If all subtowers are stable, then the tower is overall stable.
In our network, each node can be seen as representing the probability that the subtower with the block as the bottom one is stable.
We average the output of each node to get the final prediction of tower stability. The details of the graph network connectivity and output can be seen in Figure \ref{fig:graph_network}.

\begin{figure}
    \centering
    \includegraphics[clip, trim={0 0cm 0 0cm}, width=0.8\columnwidth]{figures/graph_network.png}
    \caption{(Top) The tower under consideration. (Middle) The dotted arrows on the graphs show the edges added to the graph network that correspond to the subtowers on the left. (Bottom) The output of all nodes in the graph network are averaged to get the final prediction.}
    \label{fig:graph_network}
\end{figure}

\subsection{Evaluation Tasks}
\label{sec:tasks}

We evaluate on the following downstream tasks:
\begin{enumerate}
    \item \emph{Tallest Tower:} The objective is to build the tallest possible constructable tower.
    \item \emph{Minimum Contact:} The objective is to build the tower with minimal total overlapping area between each pair of blocks.
    \item \emph{Longest Overhang:} The objective is to build the tower with the maximum distance from the center of geometry of the bottom block to the vertical side of the top block which is furthest from the bottom block. 
\end{enumerate}


==> sections/old_sections/intro.tex <==
% Original TAMP intro that focuses on local vs. global dynamics.

% TAMP Intro + General TAMP Challenges
Long horizon sequential manipulation tasks still pose a challenging problem for robotic systems. 
Tasks such as construction, assembly, and tool use involve many objects with varying physical properties. Finding a plan to achieve a task in these domains consists of reasoning in both discrete (i.e. which object to interact with, what action to take) and continuous (i.e. what motion plan to follow, where to place an object) decisions. 
A common and promising approach is task and motion planning (TAMP).
TAMP systems are specified with discrete actions, a set of objects and their properties, and samplers or optimization routines to handle decisions in continuous spaces.

% Specific TAMP Challenges we aim to address.
While TAMP systems have shown great success, many assumptions are typically made regarding the physical reasoning required to solve a problem. 
For example, it is often assumed that the dynamics of object interactions are fully known. 
However, in many scenarios, a robot may only understand a subset of the world's dynamics.
For example, a robot may have detailed models of local interactions (e.g. placing an object on a table), but not of many objects interacting with each other. 
In addition, TAMP systems are still limited by the complexity of the task at hand. 
The more objects in the environment the less tractable these solutions become.

% Example problem.
Consider a blocks world where the blocks have non-uniform mass distributions. 
In many simple pick and place domains, it may be sufficient to ignore the non-uniform mass distribution. 
\begin{figure}
    \centering
    \includegraphics[clip, trim={0 0cm 0 0cm}, width=\columnwidth]{figures/panda_intro.png}
    \label{fig:panda_intro}
    \caption{\textcolor{red}{Will get a better picture of panda constructing 5 block tower.} The Panda robot constructing a 5 block tower to improve its understanding of multiple object interactions.}
\end{figure}
However, when the blocks need to be stacked on top of each other, the robot must reason globally about the interaction dynamics between objects.
Modeling interaction dynamics presents a challenging problem for a robotics system due to the diversity of objects and their properties, as well as the combinatorially large number of ways in which they can interact.

% Our general solution (i.e., decoupling + learning) + lower level problems it introduces (sample efficiency, self-guided exploration).
To address this challenge, we introduce a system that decouples the dynamics of local and global object interactions.
We assume the robot has an accurate model of its own kinematics and local interactions in the form of a TAMP planner, but does not know how multiple objects will interact with each other.
Instead, the robot must learn a dynamics model for groups of objects by experimenting with them -- using its local model to illicit interesting behaviours to efficiently learn from.
%While this still poses a challenging learning problem due to the large joint space of robot and object states, we are able to leverage the local model to illicit interesting behaviors for the robot to efficiently learn from.

% Paragraph about the difficulty of the learning problem.
Learning global dynamics in a self-supervised manner poses a challenging learning problem due to the combinatorial input space of object states.
Randomly placing objects that interact with each other is unlikely to illicit interesting behavior.
Furthermore, this problem is exacerbated by the constraints of the physical robot and local planning system.
For example, if a single-armed manipulator can only interact with one object at a time, it is unlikely to generate interesting experiments to learn about 5-object interactions until it has learned a better model for $n$-object interactions ($n < 5$).

%This presents multiple challenges as the robot needs to generate its own data to learn about the dynamics of groups of objects of properties \emph{and} it must do so in a sample efficient manner.
%\textcolor{blue}{ NOTE: We should better explain the difficulty of having a robot generate its own dataset for multi-object interactions. To learn dynamics, we need to have a dataset that elicits all the interesting combinations of object interactions. But as we have more objects, randomly sampling joint-interactions is unlikely to lead informative examples.}

% Our high level solution. (do we need this paragraph? or is the previous sufficient?)
%The key components of the system are: (1) a TAMP planner that has known approximate dynamics for locally interacting with objects (i.e. pick and place), and (2) a learned dynamics model that predicts how multiple objects will interact with each other.
%Importantly, this dynamics model must be learned using only the local model and self-guided experimentation.
%The learning phase consists of the robot gaining experience interacting with groups of objects.
%Afterwards, the system can solve planning problems that involve complex multi-object interactions (e.g., building a tower with a large overhang), by first reasoning globally about object interactions and then planning how to manipulate each object individually.

% Deeper description of the learning solution.
%In the learning phase, the robot needs to learn a dynamics function describing how objects will interact with each other.
%Importantly, it must generate its own dataset, repeatedly causing objects to interact and observing the results.
%In order to allow for efficient learning, we develop an action-informed active learning by synthesis approach.
%At each timestep of the learning phase, the robot will choose how the objects should interact and execute this experiment using its current model.
%Additionally, the active learning is guided by the single-object TAMP planner -- when the robot imagines the possible interactions it could observe, it takes the actions from the TAMP planner into account to constrain the input space of the learner.

% maybe here we can talk about the key to getting this to work (sequential data and graph)
To enable efficient learning, we develop an action-informed active learning by synthesis approach.
At each training timestep, the robot reasons about what interactions it would most benefit from observing, then proceeds to perform this experiment using its knowledge of local object interactions.
Our key insights in this work are that:
\begin{enumerate}
\item decoupling local and global dynamics allows the robot to leverage its local model to plan experiments with complex object dynamics %that can be used for planning to achieve multiple downstream tasks,
\item during active learning, by synthesizing data from the space of actions the robot is able to take, it can generate more informative experiments that are closely tied to feasible world states the robot will encounter when planning for downstream tasks, and%(on a real robot platform?)
\item a graph network architecture inspired by the global dynamics enables generalization beyond the training data.
\end{enumerate}

We evaluate this work in a block-stacking domain, where the robot autonomously learns the global dynamics of blocks with non-uniform mass distributions.
We highlight the benefits of our active learning approach by evaluating the learned dynamics model on multiple downstream tasks.
Furthermore, the action-informed active learning, as well as the learning architecture design, improve the sample efficiency to a level where the entire learning pipeline can be performed on a real robot with minimal human intervention. 

% We propose a system which decouples TAMP solvers from the difficulties of combinatorial complexity and low-level physical reasoning, by learning a subgoal generator. The agent is able to learn the space of feasible goals through active learning and by leveraging a graph neural network. Once the subgoal generator is learned, it can be leveraged in a variety of down stream tasks.

% Experimental section/key results.
%We show that we are able to efficiently learn multi-object dynamics in a stacking domain, where the robot is tasked with interacting with blocks with non-uniform mass distributions. 
%The robot must figure out what arrangements of blocks result in stable versus unstable towers. 
%We evaluate on downstream tasks of building the tallest tower, the tower with the longest overhang, and a tower with the minimum possible contact between blocks.

% NOTE: We may need to discuss the need for learning dynamics in more detail. We kind of jump right from planning to learning. Maybe something along the lines of "As we mentioned, the space of multiple object interactions is large, thus we aim to learn the dynamics model."
% NOTE: We are vague on how the dynamics model and TAMP planner work together. Maybe we should try to be more concrete. I.e., the dynamics model proposes a plan skeleton/subgoals to the TAMP planner, which should achieve some objective (eg. tallest tower).



==> sections/old_sections/intro2.tex <==
% PI Intro about APF.

\newcommand{\apf}{{\sc apf}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\as}{(a_1, \ldots, a_n)}
\newcommand{\feas}{\phi}
\newcommand{\Feas}{\Phi}
\newcommand{\Data}{\mathcal{D}}
\newcommand{\argmin}[1]{\underset{#1}{\text{argmin}\;}}
\newcommand{\argmax}[1]{\underset{#1}{\text{argmax}\;}}
\newcommand{\A}{\mathbf{A}}
\newcommand{\ent}{\mathrm{H}}
\newcommand{\expect}[1]{\mathbb{E}_{#1}}
\newcommand{\bald}{{\sc bald}}
\newcommand{\allseq}{all sequences}
\newcommand{\sequential}{sequential}
\newcommand{\incremental}{incremental}

\students{missing high level X}

Many robot planning problems depend on being able to make accurate predictions of the dynamics of the world and the effects of the robot's interactions with the world. Detailed, physically realistic models can be expensive in terms of the training data needed to build the models, and can be computationally demanding to repeatedly evaluate.  When checking object arrangements for physical stability or feasibility of assembly, the outcome will depend both on low-level details and on the accuracy of the domain model, including properties of the objects to be manipulated, as well as the robot's motor capabilities. In general, these properties are difficult to compute reliably via physics simulation, especially within a planning loop, because of the difficulty of modeling the robot's error in basic object manipulation, the propensity of objects to stick to one another, etc. \inote{above needs reorder. the goal of this paragraph is to explain why we want to learn a model}

Learning approaches have attempted to avoid the need for an explicit planning model by learning either an end-to-end regressed model for action selection or a direct policy. While end-to-end regression and learned policies have had considerable success on specific tasks in fixed domains, they have not had as much success in generalizing easily to new, unforeseen tasks.  %Hybrid approaches combine the generalization of a compositional planning model with learned components. For example, \cite {ajay2018iros} showed an underlying coarse-grained simulator can be adjusted with data to more accurately model physical motion. Similarly, \cite{zeng2019rss} showed how a deep network could be used to predict residuals on top of control parameters predicted by a physics simulator. 
While hybrid techniques \cite {ajay2018iros,zeng2019rss} offer substantial performance improvements over unstructured models or policies, existing systems that use learned components require substantial amounts of training data, in the thousands or tens of thousands of training instances. These techniques thrive in simulation environments, where large amounts of data are readily available, but often fail in real-world robotics domains, where collecting training data is more expensive. \inote{this paragraph could also use some sharpening. the purpose is to explain the advantages of learning approaches, but also their current shortcomings}

\students{shorten above two paragraphs (less Y)}

In the process of training a model, some observations may be more valuable than others. Active learning is a technique for identifying unlabelled instances that are most informative in learning the target concept, driving down the data complexity required to achieve good performance from the learner. A robot that could identify plans whose outcomes would be informative about the underlying model, execute those plans and learn from the subsequent plan success or failure, may be able to learn with much less data than is used in the current state-of-the-art model-learning approaches. The technical challenge is how to find plans of interest --- an active learning technique requires both a way to generate candidate plans, and a way to determine how informative a candidate plan might be given the current model. \inote{good. introduces the promise and challenge of active learning}

In this paper, we describe a new approach to learning composable planning models that leverages the insight that complex robot planning problems can be most effectively addressed hierarchically: at the higher level of abstraction, the system searches over plausible abstract action sequences and then, for each abstract action, plans and possibly executes a detailed robot control plan and/or policy for motion and object interaction.  The effectiveness of this strategy hinges on our ability to learn to predict the likelihood that an action sequence will be feasible to execute. Even an approximately correct estimator of {\em abstract plan feasibility} (\apf) can offer huge computational advantages during planning.  A version of this approach is used to good effect in {\em skeleton-based} task and motion planning systems~\cite{Driess,Kim}. \inote{i think it would be helpful to say explicitly that we learn at the higher level of abstraction, and assume we have a model of the lower level dynamics}

We show how this approach to hierarchical, abstract planning can enable Bayesian active learning to train a model to predict \apf: for a given abstract action sequence, does a detailed plan exist that can be successfully executed by the robot?  In training this model, we exploit an important property of these action sequences: for an action sequence $\as$, if any prefix $(a_1, \ldots, a_i)$ is infeasible, then any longer prefix $(a_1, \ldots, a_j)$ for $i <j \leq n$ is also infeasible. \inote{This is the critical idea. in the introduction we shouldn't obfuscate it in mathematical notation unless we absolutely can't say it clearly in english}. The \apf{} properties give us leverage not only in planning but also in data acquisition for active learning. A complex plan instance may contain many elements that are highly informative for model learning, but will never be experienced because early elements in the plan will fail with high probability.

% Many difficult robot planning problems can be most effectively addressed hierarchically:  at the higher level of abstraction, the system searches over plausible abstract action sequences and then, for each abstract action, plans and possibly executes a detailed robot control plan and/or policy for motion and object interaction.   Because planning at the low level is typically very computationally expensive, we generally wish to lazily~\cite{Sidd?} postpone low-level planning until we have a complete high-level plan that we believe is likely to succeed.

\begin{figure}
    \centering
    \includegraphics[clip, trim={0 0cm 0 0cm}, width=\columnwidth]{figures/panda_intro.png}
    \label{fig:panda_intro}
    \caption{\textcolor{red}{Will get a better picture of panda constructing 5 block tower.} The Panda robot constructing a 5 block tower to improve its understanding of multiple object interactions.}
\end{figure}

% The effectiveness of this lazy strategy hinges on our ability to predict, fairly reliably, the likelihood that an action sequence will be feasible to execute.  In general, to be completely sure of plan correctness, it is necessary to find a complete plan at the primitive level using correct detailed models of the robot's interaction with the physical world.  Making a detailed plan is expensive in terms of computation and acquiring accurate physical interaction models is expensive in terms of training examples.  Happily, even an approximately correct estimator of {\em abstract plan feasibility}(\apf) can offer huge computational advantages during planning.  A version of this approach is used to good effect in {\em skeleton-based} task and motion planning systems~\cite{Driess,Kim}.

% Although in some cases it may be possible to predict \apf{} via coarse-grained simulation or, for example, checking object arrangements for physical stability or assemblability, true feasibility will depend both on low-level planning details and on the accuracy of the domain model, including properties of the objects to be manipulated, as well as the robot's motor capabilities.   In general, this cannot be computed reliably via physics simulation because of the difficulty of modeling the robot's error in basic object manipulation, the propensity of objects to stick to one another, etc.

% In this paper, we explore a strategy in which a learned model is trained to predict \apf: for a given abstract action sequence, does a detailed plan exist that can be successfully executed by the robot?  In training this model, we exploit an important property of these action sequences:  for an action sequence $\as$, if any prefix $(a_1, \ldots, a_i)$ is infeasible, then any longer prefix $(a_1, \ldots, a_j)$ for $i <j \leq n$ is also infeasible.  This {\em infeasible sub-sequence} property gives us leverage in data acquisition, learning, and planning.

We apply this active learning strategy to the concrete problem of stacking blocks, with non-uniform mass distributions whose centers of mass are approximately known, into towers satisfying several different objective functions (including the tallest possible tower or the tower with maximal overhang) using a real Panda Emika robot arm, illustrated in figure~\ref{fig:panda_intro}. \inote{re-word so it doesn't seem like we have the objective functions at train time}.  The robot designs, plans, and executes experiments completely autonomously with a set of objects and learns an \apf{} predictor; within the setting of block assemblies, it identifies the most informative plans for \apf{}, attempts to execute these plans and then uses the resulting plan success or failure as a label for the training instance.  The learned plan predictor can then be used within the planning loop to plan efficiently for different objectives using different sets of objects.  This efficient autonomous learning process relieves engineers from tedious work in supervising and resetting the experimental environment and results in a highly flexible and robust system for planning and executing complex action sequences in the real world.

%The \apf{} test must be learned from data acquired from attempted detailed planning and execution for a set of abstract plans.  Because robot experience is very expensive to gather, we focus aggressively on reducing the amount of data required and the ease of acquiring it.  Our strategy includes:

Our contributions include: 
\begin{itemize}
    \item An active learning approach to select test plans that are as informative as possible; 
    \item A  neural network model to have inductive bias appropriate to the structure of the prediction problem; and 
    \item Autonomous self-supervised experiment execution via an integrated perception, learning, experimentation, planning, and execution loop.
\end{itemize}

%We apply this strategy to the concrete problem of stacking objects, with non-uniform mass distributions whose centers of mass are approximately known, into towers satisfying several different objective functions (including the tallest possible tower or the tower with maximal overhang) using a real Panda Emika robot arm, illustrated in figure~\ref{fig:panda_intro}.  The robot designs, plans, and executes experiments completely autonomously with a set of objects and learns an \apf{} predictor;  then using that predictor it plans efficiently to satisfy different objectives using different sets of objects.  This efficient autonomous learning process relieves engineers from tedious work in supervising and resetting the experimental environment and results in a highly flexible and robust system for planning and executing complex action sequences in the real world.


%Active experimentation
%One way to formulate the active experimentation problem is at the level of assemblies:  following submodular blah blah, we select the assembly that will be the most informative and attempt to build it, observing whether it is successful or not.

%Some stuff about using an ensemble of neural nets to represent uncertainty, etc.

%However, there is an important piece of prior information that applies to many sequential assembly problems, which is that if any subsequence of the assembly is not feasible, then the whole structure will not be feasible.  It is difficult to build this prior into the neural network predictor.

%Instead, we build it into our information-gathering strategy and so, rather than considering the most informative of all possible assemblies, we consider the most informative assembly that consists of a single step beyond an assembly we already know is feasible.

%An additional important observation is that our selection of the next experiment to try does not take into account the expense of actually building the assembly.   Consider the case where the robot has conjectured a 3-part assembly and built it successfully.  The most informative next assembly might be completely different from this one, requiring the robot to disassemble the current assembly and then build the new one.   An alternative is to be opportunistic:  given that the robot has a newly built assembly, it can very cheaply gain additional information by making the most informative addition to the current assembly.




==> sections/old_sections/method.tex <==
\begin{figure}
    \small
    \includegraphics[trim={0 0 0 0},clip,width=.99\columnwidth]{figures/method_overview.png}
    \caption{Overview of our method, described in Section \ref{sec:method}}
    \label{fig:method_overview}
\end{figure}

\subsection{Learning}

We aim to learn a model which is able to make predictions in sequential decision-making problems involving multiple objects. 
Our current work is limited to classification predictions, but could be extended to handle regression.
The model, $p(\bm{y} | \bm{x} ; \bm{\theta})$, takes as input the state of the objects, $\bm{x}$, and returns a prediction $\bm{y}$, determined by the parameters of the model, $\bm{\theta}$.
We also maintain a posterior distribution over our model parameters given the data we have seen so far, $p(\bm{\theta}|D)$, by leveraging an ensemble of models, which we discuss in Section \ref{sec:bald}.
The learning process occurs in several repeating steps.

First, the robot synthesizes a pool of potential inputs, $D_{pool}$ (shown in blue in Figure \ref{fig:method_overview}).
In the case of multiple object interactions, the size of this space makes random data acquisition unlikely to succeed.
In our work we are able to handle this by only considering inputs to the model that differ from data already seen by one action.
This prevents the agent from considering full inputs that it is incapable of actually attempting.
We elaborate on this in Section \ref{sec:acquisition}.

Next, we find the inputs, $D_{BALD}$, from $D_{pool}$ that will maximally reduce the entropy over our model parameters, $H(\bm{\theta}|D)$, when labeled, by using the BALD \cite{houlsby_bayesian_2011} objective (shown in red in Figure \ref{fig:method_overview}).
This objective selects inputs which our model is uncertain about, and which result in high disagreement across our ensemble predictions.
This is discussed in more detail in Section \ref{sec:bald}.

Now that we know which inputs would most benefit our model, we need to label them (shown in orange in Figure \ref{fig:method_overview}).
Here we are able to leverage our TAMP planner by giving it our desired object states, $\bm{x}$.
The robot then executes the returned plan, and labels the input with its associated $\bm{y}$.

Finally, the model parameters can be updated given the newly received labelled data, $D_{train}$ (shown in green in Figure \ref{fig:method_overview}), and the cycle repeats.

\subsection{Evaluation}

The benefit of learning a global model is that it can be used for several downstream tasks. 
To evaluate the performance of our model, we supply a task-specific objective function, $f_{task}$, and the ground truth optimal value of this function, $v_{gt}$.
We then optimize this objective function, subject to the desired constraint of the model, to find the optimal input, $\bm{x}_{opt}$ (shown in purple in Figure \ref{fig:method_overview}).
Then, we pass the desired state, $\bm{x}_{opt}$, to the TAMP planner to get an executable plan to attempt to achieve this state. 
Finally, we execute the plan and determine the true value of the given state, $v_{opt}$.
The metric we use to evaluate performance is regret, or the difference between the ground truth optimal value, $v_{gt}$, and the value found when using our model, $v_{opt}$.
If we have learned a good model that is representative of the phenomena we are aiming to characterize, this value should approach the ground truth optimal value, and our regret will approach zero.

==> sections/old_sections/method2.tex <==
There are two distinct phases in the operation of our system, as illustrated in figure~\ref{fig:method_overview}: in the {\em experimentation phase}, the robot ``curiously'' plays with the objects available to it, learning an \apf{} model;  in the {\em execution phase}, the robot is given novel objects and goals to achieve, and it uses the learned \apf{} model to efficiently plan successful action sequences.   In this section, we describe our formulation and approach to each of these problems.

\subsection{Problem Formulation}
\label{sec:exp-design}
Our objective is to learn a model that predicts plan success, that is, to learn the parameters $\Theta$ that most accurately predict 
\[
\Pr(\phi \mid \ba; \Theta),
\]
where $\phi \in \{0, 1\}$ is the success of the plan given by action sequence $\ba \in \A$. We wish to learn $\Theta$ from a sequence of data $\Data$, and we wish to learn $\Theta$ from a minimal length sequence of $\Data$. 

  %Although our problem is not precisely sub-modular, in ways we will discuss later in this section, we will nonetheless pursue a greedy strategy for selecting experiments. 
%Our space of possible experiments is the space of action sequences $\A$.  
%We begin by describing how we select among a given set $\A$, and then explore different choices of the set $\A$.  

\subsubsection{Entropy reduction}
Following \ref{Mackay92,Cohn96}, we can pick a sequence of data $\Data$ that maximizes the information gain, or reduces the entropy of $\Pr(\Theta \mid \Data)$. The general problem of designing a sequence of experiments to maximize some sort of information gain is a difficult sequential decision-making problem.  In many cases, due to sub-modularity of the objective, a greedy, ``myopic'' approach that considers only the next experiment to conduct can be shown to be a good approximation to the optimal experimentation strategy~\cite{Krause?}. 

Given a model distribution $\Pr(\Theta \mid \Data)$ that depends on the data we have seen so far, $\Data$, we choose the $\ba \in \A$ that reduces the entropy of the posterior distribution as much as possible: \inote{this seems to imply that we've already marginalized out $\phi$? I think we need to put that back in}
\begin{equation}\label{eq:theta_entropy_objective2}
\ba^* = \argmin{\ba\in\A} \ent(\Theta \mid \Data, \ba)\;\;. 
\end{equation}
While the agent can select the action sequence to experiment with, $\ba$, it cannot select the outcome $\feas$, so to compute this quantity, we have to take an expectation over the outcome, using our current model distribution:
\[\ent(\Theta \mid \Data, \ba) = \expect{\feas \sim \Pr(\cdot \mid \Data, \ba)} \ent(\Theta \mid \Data, \ba, \feas) \;\;,\]
where 
\[\Pr(\feas \mid \Data, \ba) = \int_\theta \Pr(\feas \mid \ba; \theta) \Pr(\theta \mid \Data)\;\;.\]

Estimating the entropy over a high-dimensional parameter space is difficult, so we follow the approach of~\citet{houlsby_bayesian_2011} to reformulate the objective in (\ref{eq:theta_entropy_objective2}) as 
\begin{equation}\label{eq:y_entropy_objective2}
\ba^* = \argmax{\ba\in\A} \ent(\Feas \mid \Data, \ba) - 
                          \expect{\theta \sim \Pr(\cdot \mid \Data)} \ent(\Feas \mid \ba; \theta)\;\;,
\end{equation}
allowing the computation of entropies to take place in the typically lower-dimensional label space. This is known as the \bald{} objective. \inote{is the switch between $\theta, \Theta$ or $\phi, \Phi$ supposed to represent a specific value vs a random variable?}

In addition to improved efficiency, the objective in (\ref{eq:y_entropy_objective2}) invites an appealing interpretation: maximizing the first term encourages selecting an $\ba$ that our model is overall uncertain about, and minimizing the second term encourages selecting an $\ba$ for which the individual models $\theta$ can make confident predictions about the outcome $\feas$.  If we think of the overall uncertainty as a combination of epistemic and aleatoric uncertainty, then this objective seeks an example with high overall uncertainty and low aleatoric uncertainty, which therefore has high epistemic uncertainty.  In other words, if the various possible models in $\Pr(\Theta \mid \Data)$ are individually confident but about differing outcomes, then observing the $\feas$ value corresponding to $\ba$ is likely to prove some of those outcomes incorrect. 
Using an ensemble of equally weighted parameter vectors $\theta_1, \ldots, \theta_N$ to represent $\Pr(\Theta \mid \Data)$ allows us to compute a global feasibility prediction
\[
\widehat{\Pr}(\Feas = \feas \mid \ba; \theta) = \frac{1}{N} \sum_{i=1}^N \Pr(\Feas = \feas \mid \ba; \theta_i)
\]
as well as find the experiment that optimizes the estimated \bald{} objective in the form \begin{equation}\label{eq:final-criterion}
\ba^* = \argmax{\ba\in\A} \ent(\widehat{\Pr}(\Feas \mid \ba; \theta)) - 
                          \frac{1}{N}\sum_{i=1}^N \ent(\Pr(\Feas \mid \ba; \theta_i))\;\;.
                          \end{equation}
\subsection{Abstract plan feasibility model}
\label{sec:method-apf-model}
The role of the \apf{} model is to predict the probability that an action sequence is feasible, $\Pr(\feas \mid \ba)$, where $\ba = \as$ is an action sequences, $\feas$ is a Boolean random variable indicating that the action sequence can be executed feasibly, and the probability distribution represents inherent {\em aleatoric uncertainty} due to unmodeled behavior of the detailed planning process and execution of actions in the world.

\begin{figure*}
\includegraphics[width=0.95\linewidth]{figures/overview.png}
\caption{\label{fig:method_overview} The proposed system that learns \emph{Abstract Plan Feasibility} (\apf{}) operates in two phases. \textbf{Experimentation Phase} (left) First, the robot will iteratively design and execute experiments that improves its \apf{} model. (A) Using its current model, the robot selects the action sequence, $\mathbf{a^*}$ that minimizes its entropy over \apf{} models. (B) The robot computes and executes a detailed motion plan for executing the abstract action sequence. (C) After observing the true plan feasibility, $\phi$, the robot updates its \apf{} model, represented as an ensemble of neural networks. \textbf{Execution Phase} (right) Once an \apf{} model has been learned, the robot can use it to perform various tasks, such as build the tallest tower, or the tower with the largest overhang.}
\end{figure*}

Because our objective is to learn the \apf{} model from as few data samples as possible, it is critical that it be formulated in a way that makes our {\em epistemic uncertainty} about the model explicit.  We do this by representing a particular model using a parameter vector $\theta$ in the space of possible \apf{} models $\Theta$.  So the prediction of a particular model is $\Pr(\feas \mid \ba; \theta)$ and our epistemic uncertainty can be described in terms of a distribution on the model parameter space, $\Pr(\Theta)$.

In general, for complex model classes, explicit representation and updating of $\Pr(\Theta \mid \Data)$ for training data $\Data$ is too difficult.  We follow the strategy of~\citet{ensemble} and represent this uncertainty using an ensemble of $k$ models, whose initial parameters $(\theta_1, \ldots, \theta_k)$ are drawn independently at random and are updated to incorporate new data via gradient descent.

The design of the models in the ensemble is selected to match the underlying structure of the prediction problem.  Importantly, the length of action sequences for which we require predictions varies during both the experimentation and execution phases.  For this reason, we use {\em graph neural networks} ({\sc gnn}s), which make predictions based on aggregations of local properties and relations among the input entities, and exploit parameter tying to model global properties of collections of objects of arbitrary size using a fixed-dimensional parameterization $\Theta$.  For a detailed description of {\sc gnn}s, see the overview by \citet{Battaglia}.

We take advantage of the {\em infeasible sub-sequence} property of the \apf{} problem to design a special connectivity structure for our {\sc gnn} models.  As shown in figure~\ref{fig:graph_network}, the node corresponding to action $a_i$ is connected to each node representing $a_j$ for $1 \leq j < i$.  This encodes the structural property that the feasibility of step $i$ in the plan depends on all previous actions.  To make a prediction, an encoding of $\ba$ is fed into the network, some number of rounds of message passing is performed on the graph using the local neural network models $\theta$, and the average activation level of each node is computed and passed through a sigmoidal transformation to obtain a prediction $\Pr(\feas \mid \ba)$.

\lpknote{We might want to put more details in here?}



\subsubsection{Domain of experimentation}
Now that we have established a strategy for selecting the best experiment from a set $\A$, we investigate several choices of that set.   Let $\mathcal{A}$ be a (possibly infinite) set of possible individual actions and $L$ be the maximum action-sequence length.  

Most straightforwardly, we would let $\A$ be all possible sequences $(a_1, \ldots, a_l)$ with $a_i \in \mathcal{A}$ and $1 \leq l \leq L$. 
We not be able to maximize objective (\ref{eq:final-criterion}) over the entire set and will therefore have to let $\A$ be a randomly generated set of samples from that space and optimize only over the samples.   We call this the {\it \allseq{}} strategy.

The \allseq{} approach might generate most of its samples in the infeasible part of the space, requiring a large sample set and causing slow computation.
We observe that the infeasible sub-sequence property provides a strong constraint on the set of actually feasible action sequences:  sequence $\as$ is only feasible if all of its prefixes are also feasible.  We can use this insight to bias our sampling to focus on action sequences that are much more likely to be feasible by only considering sequences $\as$ for which the prefix $(a_1, \ldots, a_{i-1})$ together with result $\feas = 1$ are in the current data set $\Data$.  We call this the {\it \sequential{}} strategy.

Finally, we observe that asking the robot to execute action sequences is a substantial cost and that if it has just finished successfully executing a sequence $\as$, rather than asking for a completely unrelated sequence, we have the opportunity to immediately append another action to that sequence and execute just the last step on the robot.  In this {\em \incremental{}} strategy, we let $\A$ consist only of one-step continuations of the previous action sequence if it was feasible, and otherwise revert to the \sequential{} approach.

\subsection{Integrated system}

In this section, we illustrate the integration of the active learning methodology into an overall experimentation, learning, planning, and execution system, which operates in two phases:  experimentation and execution.  

Both phases depend on the ability to construct and execute detailed plans on a real robot given an abstract action sequence.  We assume that a detailed planning and execution system is available that can integrate perception, planning, and control to carry out that action sequence and observe whether or not it was successful.  In section~\ref{experimentPlanner} we describe our experimental implementation of such a system in detail.  In the following, we assume the existence of a procedure \textproc{detailedPlanEx}, which takes a sequence of abstract actions $\ba$ and the current robot state, and performs closed-loop perception, planning, and control to execute actions $a \in \ba$ in sequence until it determines that $\ba$ has been successfully carried out or has become impossible.  It returns a Boolean value indicating whether it succeeded.

\subsubsection{Experimentation phase}
The experimentation phase operates, as shown in algorithm~\ref{exper_pseudocode}, as follows.  It starts by initializing $n_m$ separate parameter sets $\theta$ for the {\sc gnn}s representing the $\apf$ model.  It then iterates $n_i$ through an experimentation and training loop.  It is parametrized by an action sampling strategy (one of \allseq{}, \sequential{}, or \incremental{}), which it uses to generate $n_s$ sample action sequences $A_hat$ (note that the \incremental{} strategy depends on the current world state and is really only sensible for $n_b = 1$).  Then, the approximate \bald{} objective is used to select the best batch of $n_b$ action sequences $A_batch$ from $A_hat$.  These action sequences are executed, yielding results $\phi_batch$, and the test sequences and results are added to the data set.  Finally, the parameters $\theta_i$ for each model in the ensemble are updated and a new iteration begins.

\begin{scriptsize}
\begin{verbatim}
    explore(n_b, n_s, n_m, n_i, A, L, sampler, world_state)
        Theta = (\theta_1, \ldots, \theta_n_m) randomly initialized GNNs
        D = {}
        for iteration in n_i
            A_hat = sampler(A, L, D, n_s, world_state)
            A_batch = top_n(bald(., Theta), A_hat, n_b)
            Phi_batch = [detailedPlanEx(a, world_state) for a in A_batch]
            D = D u zip(A_batch, Phi_batch)
            Theta = [train(theta, D) for theta in Theta]
        return Theta
\end{verbatim}
\end{scriptsize}
\lpknote{If this pseudocode is worth having, then typeset}

\subsubsection{Execution phase}

After the \apf{} model has been learned, it can be used flexibly to achieve multiple objectives.  We assume that the robot is given an objective function $V$ which maps action sequences to real values and its goal is to find an abstract action sequence 
\[\ba^*= \argmax{\{\ba \in \A \mid \Pr(\feas \mid \ba) > 1-\epsilon\}} V(\ba)\;\;,\]
which has high value subject to being $1-\epsilon$ likely to be feasibly executable.

\lpknote{Add some detail here about the Monte-carlo planner we are using to select plans at performance time.}

==> sections/old_sections/old_bald.tex <==

We represent each observed interaction with the world by an initial state $\bm{x}_i \in \mathcal{X}$ and an observed outcome $\bm{y}_i \in \mathcal{Y}$. The collection of all observations is our training data: $\mathcal{D} = \{(\bm{x}_1, \bm{y}_1), (\bm{x}_2, \bm{y}_2),  \dots\}$. Our objective is to learn the transition dynamics $p(\bm{y} | \bm{x} ; \bm{\theta})$  with parameters $\bm{\theta}$ in as few interactions as possible.

Denoting the posterior distribution over our parameters given our observations by $p(\bm{\theta} |\mathcal{D})$, we formalize our ``few interactions'' objective as selecting observations which maximally reduce the uncertainty over $p(\bm{\theta} |\mathcal{D})$, quantified by Shannon entropy $H(\bm{\theta} | \mathcal{D})$. This can also be seen as selecting interactions which reduce the the size of the hypothesis space as quickly as possible.

\begin{equation}
    \underset{\mathcal{D}}{\text{argmin}} \  H(\bm{\theta} | \mathcal{D})
\end{equation}

While finding the set of interactions that jointly minimize the entropy of the parameters is difficult, entropy is submodular and monotone, which means that a greedy sequential selection will be within $(1 - \frac{1}{e})$ of optimal \cite{Nemhauser1978submodular}. 

\begin{equation}
    \underset{\bm{x}, \bm{y}}{\text{argmax}} \  H(\bm{\theta} | \mathcal{D}) - H(\bm{\theta} | \bm{x}, \bm{y}, \mathcal{D})
\end{equation}

While the agent can put the world in an initial state $\bm{x}$, it cannot select the outcome $\bm{y}$. Fortunately, we have a prediction of $\bm{y}$ using our learned dynamics dynamics:

\begin{equation}
    \underset{\bm{x}}{\text{argmax}} \  H(\bm{\theta} | \mathcal{D}) - \mathbb{E}_{\bm{y} \sim p(\cdot | \bm{x}, \mathcal{D})}  \left [ H(\bm{\theta} | \bm{x}, \bm{y}, \mathcal{D}) \right ]
    \label{eq:theta_entropy_objective}
\end{equation}

Computing entropy is subject to the curse of dimensionality.  dimensionality, and the parameter space is often high-dimensional. To address this, Houlsby et. al. \cite{houlsby_bayesian_2011} show that Equation \ref{eq:theta_entropy_objective} is equivalent to 

\begin{equation}
    \underset{\bm{x}}{\text{argmax}} \  H(\bm{y} | \bm{x}, \mathcal{D}) - \mathbb{E}_{\bm{\theta} \sim p(\cdot |\mathcal{D})}  \left [ H(\bm{y} | \bm{x}, \bm{\theta}) \right ]
    \label{eq:y_entropy_objective}
\end{equation}

 allowing the computation of entropies in the typically lower-dimensional label-space. In addition to saving compute, Equation \ref{eq:y_entropy_objective} invites an appealing interpretation: the left term encourages selecting an $\bm{x}$ such that our model is overall uncertain of the outcome, $\bm{y}$, and the right term encourages selecting an $\bm{x}$ such parameters sampled from the posterior are confident of the outcome. In other words, the various possible models in the posterior distribution over $\bm{\theta}$ are individually confident but about differing outcomes, and observing $\bm{y}$ is therefore likely to prove some of those outcomes incorrect.


==> sections/old_sections/old_intro.tex <==
%manipulation on a real robot and why it's hard: want to learn a model on the real robot as it incorporates real work phenomena. 

Models are used in robotic manipulation tasks to enable a robot to reason about how to achieve a goal.
These models approximate reality and have many assumptions baked in to them.
For example, one may assume that, regardless of the properties of an object (eg. shape, center of mass, deformability), when it is placed on a surface it will remain stably resting there.
Physics-based simulators can also be used as models and thus the model takes on the approximations of the simulator.
These include things like penetrating contact surfaces and simplified friction dynamics.
In order to achieve better performance on real-world manipulation tasks, we need models that are better at representing real world phenomena and stochasticity.
Things like the contact force exerted when an object is placed on another, or the effects of an object's mass distribution on how it moves when in contact, or even the interaction between a robot's gripper and an object it is placing can be very challenging to model. 
However, accurately modeling these can have a big impact on the success of a task.

%how do we do that? given limitations of data collection?  typically things have to be modelled, but learning is a means to be more general

One way to address this challenging modeling problem is to learn the model through real world robot interactions.
Learning systems provide a general way to capture real world phenomena under a single method, without having to use an analytical model of each  (eg. stability, dynamic motions, contact, etc..) separately.
However, learning systems are notoriously data inefficient, and data collection on a real system is expensive in term of the time it takes to collect data.
In addition, it is often unclear what the structure of the learned model should be to enable efficient learning and generalizability.

%in this paper we develop a method which is able to learn a model that can be used to solve several downstream tasks (And we can use our model for different downstream tasks.)via planning, with all training data collected on the robot. we achieve this through active learning and a graph network

In this work we present a learning system which is able to collect real-world robot data, train a model, and use that model for several downstream manipulation tasks. The key ideas that enable this work are:
\begin{enumerate}
    \item \textit{Active Learning:} To address the data efficiency issue, we guide data collection by enabling the robot to select and construct new training data interactions by reasoning about what data would most reduce the uncertainty of its predictions.
    \item \textit{Graph Network:} We design a graph neural network which takes inspiration from the problem space at hand. We show that by incorporating insights from the known structure of this space, we can be much more data efficient. This structure, along with weight sharing on the nodes and edges of the graph network, allows the robot to generalize training data to novel scenarios.
\end{enumerate}

%domain and hint at results/what we will show in the evaluation

We evaluate this method in the towers domain. Here the robot learns a model which is able to predict whether or not a given tower of blocks with non-uniform density is constructable.
Given a set of novel blocks not seen during training, we show that this model can be used to plan for the tallest possible tower, deconstructing a tower without any blocks falling, and building a tower with the longest overhang.
We also show the benefits of active data acquisition and the custom graph network in vastly reducing the required data, and making real-world model learning feasible.


\subsection{Notes from meeting}

What priors are we bringing into our curiosity framework?

\begin{enumerate}
    \item Stable states (we're curious about whether the built towers fall over)
    \item Sequential building (place one block at a time)
    \item The structure of the computation (GNN)
\end{enumerate}
